GPU-Accelerated WFST Beam Search Decoder for CTC-based Speech Recognition

While Connectionist Temporal Classification (CTC) models deliver state-of-the-art accuracy in automated speech recognition (ASR) pipelines, their performance has been limited by CPU-based beam search decoding. We introduce a GPU-accelerated Weighted Finite State Transducer (WFST) beam search decoder compatible with current CTC models. It increases pipeline throughput and decreases latency, supports streaming inference, and also supports advanced features like utterance-specific word boosting via on-the-fly composition. We provide pre-built DLPack-based python bindings for ease of use with Python-based machine learning frameworks at https://github.com/nvidia-riva/riva-asrlib-decoder. We evaluated our decoder for offline and online scenarios, demonstrating that it is the fastest beam search decoder for CTC models. In the offline scenario it achieves up to 7 times more throughput than the current state-of-the-art CPU decoder and in the online streaming scenario, it achieves nearly 8 times lower latency, with same or better word error rate.

==> junk.tex <==
\begin{figure}[h!]
\begin{algorithm}[H]
\algrenewcommand{\algorithmiccomment}[1]{\hskip1em$\#$ \footnotesize#1 \normalsize}
\small
\hspace*{2.5em} $k$: beam size, \ $M$: maximum length, \\
\hspace*{2.5em} $\vocab$: Vocabulary, \
 $\score(\cdot)$: scoring function.
\begin{algorithmic}[1]
\State $B_0 \gets \{ \langle 0, \bos \rangle \}$
\For{ $t \in \{ 1, \dots, M\!-\! 1 \}$ }
    \For{$ \langle s, \rvy \rangle \in B_{t-1}$}
     \If{\ $\rvy.\mathrm{last}() = \eos$}

      \State \colorbox{red!15}{$H.\mathrm{add}(\langle s, \rvy \rangle )$} \label{line:vanilla_h}
      \State \textbf{continue}
    \EndIf
    \For{$y \in \vocab$}
        \State $s \gets \score(\rvy \circ y)$,
        \ $H.\mathrm{add}( \langle s, \rvy \circ y \rangle)$
    \EndFor
    \EndFor
    \State  $B_t \gets \varnothing$
\While{$ |B_t| < k $} \algorithmiccomment{Find top $k$ from $H$.}
\small \State $ \langle s, \rvy \rangle \gets H.\mathrm{max}()$, $B_t.\mathrm{add}(\langle s, \rvy \rangle)$
\State $H.\mathrm{remove}(\langle s, \rvy \rangle)$
\EndWhile

 \hspace*{-\algorithmicindent} \hspace*{-\algorithmicindent} \hspace*{-2\fboxsep}\colorbox{green!25}{\parbox{1.0\linewidth}{\If{$\rvy.\mathrm{last}() = \eos\
$, $\forall \rvy \in B_t$}\algorithmiccomment{All finished.}\EndIf}} \label{line:vanilla_stop}
 \vspace*{-0.3cm}
\State  \hspace*{\algorithmicindent} \Return $B_t.\mathrm{max}()$
\EndFor
\State \Return $B_t.\mathrm{max}()$

\end{algorithmic}
\caption*{\small \textbf{Vanilla Beam Decoding}}
\end{algorithm}
\caption{The vanilla version of beam decoding. The top-$k$ operation is applied over $H$, the union of the finished and continuing sequences. This is implem\
ented, for example, in the TensorFlow Addons library \cite{tensorflow2015-whitepaper}.\protect\footnotemark{}
See also \citet{stahlberg-byrne-2019-nmt,meister-etal-2020-best}.
}
\label{alg:vanilla}
\end{figure}

